Evidence for bimodal orbital separations of white dwarf-red dwarf binary stars

We present the results of a radial velocity survey of 20 white dwarf plus M dwarf binaries selected as a follow up to a \textit{Hubble Space Telescope} study that aimed to spatially resolve suspected binaries. Our candidates are taken from the list of targets that were spatially unresolved with \textit{Hubble}. We have determined the orbital periods for 16 of these compact binary candidates. The period distribution ranges from 0.14 to 9.16\,d and peaks near 0.6\,d. The original sample therefore contains two sets of binaries, wide orbits ($\approx100-1000$\,au) and close orbits ($\lesssim1-10$\,au), with no systems found in the $\approx10-100$\,au range. This observational evidence confirms the bimodal distribution predicted by population models and is also similar to results obtained in previous studies. We find no binary periods in the months to years range, supporting the post common envelope evolution scenario. One of our targets, WD\,1504+546, was discovered to be an eclipsing binary with a period of 0.93\,d.

==> alias_table.tex <==


\begin{table}
  \caption{Fitted periods and aliases shown with the corresponding reduced $\chi^2$ value. For each target, the number of valid data points, N, used in the analysis is also shown.}
  \begin{tabular}[width=\textwidth]{ c  l  l  l  l  l  }
    \hline
    WD & N  & alias  & Period  & $\chi^2$ & $\chi^2_{red}$ \\
       &    &        &  (days) &		  & \\
    \hline
     0023$+$388  & 16 & 1 & 1.87741(7)  & 41.95 & 2.9 \\
                 &    & 2 & 0.642599(6) & 42.76 & 3.0 \\
                 &    & 3 & 0.677711(8) & 54.07 & 3.9 \\
%    0145$-$221 & 0.41583      & -      & -      & -     & 11 600 & 8.10 & 0.74(3) & L     & 2,3,4,5  \\
     0303$-$007  & 31 & 1 & 0.541136(3) & 195.98 & 7.3 \\
                 &    & 2 & 1.191022(2) & 957.83 & 35.5 \\
     0354$+$463  & 49 & 1 & 0.1652026(4)& 73.53  & 1.6 \\
				 &    & 2 & 0.2468960(9)& 468.84 & 10.4\\
     0430$+$136* & 30 & 1 & 0.1063487(2)& 28.22  & 1.1 \\
     0752$-$146  & 21 & 1 & 1.049449(9) & 54.21  & 3.2 \\
                 &    & 2 & 0.522410(5) & 93.46  & 5.5 \\
     0812$+$478* & 16 & 1 & 0.118414(6) & 7.96   & 0.6 \\
                 &    & 2 & 0.217832(7) & 7.99   & 0.7 \\
     0908$+$226  & 26 & 1 & 9.1584(3)   & 30.32  & 1.4 \\
                 &    & 2 & 8.9426(3)   & 33.37  & 1.5 \\
                 &    & 3 & 0.90155(3)  & 45.29  & 2.1 \\
     1001$+$203* & 22 & 1 & 0.0558312(7)& 7.48   & 0.4 \\
                 &    & 2 & 0.0528475(7)& 8.45   & 0.5 \\
     1037$+$512  & 22 & 1 & 0.141403(1) & 61.47  & 3.4 \\
                 &    & 2 & 0.165068(2) & 68.40  & 3.8 \\
                 &    & 3 & 0.123758(1) & 82.98  & 4.6 \\                 
     1051$+$516  & 22 & 1 & 2.77007(5)  & 72.99  & 4.0 \\
                 &    & 2 & 0.2651658(7)& 346.94 & 19.2\\
     1133$+$358  & 19 & 1 & 5.9559(4)   & 13.41  & 0.9 \\
                 &    & 2 & 6.05516(4)  & 17.86  & 1.2 \\
     1333$+$487  & 10 & 1 & 0.57864(4)  & 30.69  & 5.1 \\
                 &    & 2 & 0.365456(5) & 39.21  & 6.5 \\
     1339$+$606  & 13 & 1 & 0.49234(1)  & 11.97  & 1.3 \\
                 &    & 2 & 0.99031(9)  & 13.57  & 1.5 \\
                 &    & 3 & 0.33082(2)  & 16.30  & 1.8 \\
     1433$+$538  & 21 & 1 & 4.4794(1)   & 23.69  & 1.4 \\
                 &    & 2 & 4.3565(1)   & 25.25  & 1.5 \\
                 &    & 3 & 4.6068(1)   & 33.09  & 1.9 \\
     1436$-$216  & 32 & 1 & 2.0177(2)   & 58.21  & 2.1 \\
                 &    & 2 & 0.66987(2)  & 73.57  & 2.6 \\
     1458$+$171  & 11 & 1 & 0.164702(8) & 8.90   & 1.3 \\
                 &    & 2 & 0.246086(2) & 9.60   & 1.4 \\
     1504$+$546  & 39 & 1 & 0.930722(6) & 175    & 5.0  \\ 
                 &    & 2 & 0.479531(2) & 880    & 25.1 \\
     2257$+$162  & 14 & 1 & 0.3228(7)   & 19.34  & 1.9  \\ 
                 &    & 2 & 0.4735(3)   & 77.98  & 7.8 \\
%    1517$+$502 & -            & -      & -      & ?     & 31 100 & 7.84 & -       & dC    & 1,2 \\
     2317$+$268  & 12 & 1 & 0.7944(9)   & 25.10  & 3.1  \\ 
                 &    & 2 & 0.4425(3)   & 37.06  & 4.6 \\
%    2317$+$268 & 0.7944(9)    & 132(3) & 13(2)  & DA1.6 & 31 500 & 7.70 & 0.52(2) & dM3.5 & 1,2,3 \\
    \hline
  \end{tabular}
  \label{tab:periods}
\end{table}


==> distancetable.tex <==

\begin{table}
  \caption{White dwarf temperature and log g from the literature.}
  \begin{tabular}{ c  c  c  l  l l }
    \hline
    WD & Teff       & log g        & Mass & Distance & Ref \\
       & (K)        &              &      & (pc)     &     \\
  \hline
    0023$+$388 & 10980[164] & 8.21[0.05] & 0.73[0.03] & 56  & 1 \\
    0145$-$221 & 12150[180] & 8.21[0.05] & 0.74[0.03] & 47 & 1 \\
    0303$-$007 & 17050[327] & 7.77[0.06] & 0.49[0.03] & 125 & 1 \\
    0354$+$463 & 8240[126]  & 7.96[0.10] & 0.57[0.06] & 34 & 1 \\
    0430$+$136 & 34210[614] & 8.07[0.09] & 0.69[0.05] & 209 & 1 \\
    0752$-$146 & 19440[291] & 7.92[0.04] & 0.58[0.02] & 37 & 1  \\
    0812$+$478 & 62000[1195]& 7.63[0.06] & 0.57[0.02] & 246 & 1 \\
    0908$+$226 & -          & -          & -          & -   & \\
    1001$+$203 & 21010[439] & 7.88[0.06] & 0.56[0.03] & 93 & 1 \\
    1037$+$512 & 19780[346] & 7.99[0.05] & 0.62[0.03] & 124 & 1 \\
    1051$+$516 & -          & -          & -          & - &  \\
    1133$+$358 & -          & -          & -          & - &  \\
    1333$+$487 & -          & -          & -          & - &  \\
    1339$+$606 & 44770[1043]& 7.75[0.09] & 0.57[0.04] & 407 & 1 \\
    1433$+$538 & 23260[379] & 7.82[0.05] & 0.54[0.02] & 149 & 1 \\
    1458$+$171 & 22600[490] & 7.45[0.07] & 0.40[0.02] & 214 & 1\\
    1504$+$546 & 23120[464] & 7.88[0.06] & 0.56[0.03] & 136 & 1\\
    1517$+$502 & -          & -          & -          & -   & \\
    2257$+$162 & 25450[396] & 7.54[0.05] & 0.45[0.02] & 207 & 1\\
    2317$+$268 & 31890[486] & 7.71[0.06] & 0.52[0.02] & 243 & 1\\
    
    \hline
  \end{tabular}
  \label{tab:spectroscopy}
\end{table}

